A Unified Evaluation of Textual Backdoor Learning: Frameworks and Benchmarks

Textual backdoor attacks are a kind of practical threat to NLP systems. By injecting a backdoor in the training phase, the adversary could control model predictions via predefined triggers. As various attack and defense models have been proposed, it is of great significance to perform rigorous evaluations. However, we highlight two issues in previous backdoor learning evaluations: (1) The differences between real-world scenarios (e.g. releasing poisoned datasets or models) are neglected, and we argue that each scenario has its own constraints and concerns, thus requires specific evaluation protocols; (2) The evaluation metrics only consider whether the attacks could flip the models' predictions on poisoned samples and retain performances on benign samples, but ignore that poisoned samples should also be stealthy and semantic-preserving. To address these issues, we categorize existing works into three practical scenarios in which attackers release datasets, pre-trained models, and fine-tuned models respectively, then discuss their unique evaluation methodologies. On metrics, to completely evaluate poisoned samples, we use grammar error increase and perplexity difference for stealthiness, along with text similarity for validity. After formalizing the frameworks, we develop an open-source toolkit OpenBackdoor to foster the implementations and evaluations of textual backdoor learning. With this toolkit, we perform extensive experiments to benchmark attack and defense models under the suggested paradigm. To facilitate the underexplored defenses against poisoned datasets, we further propose CUBE, a simple yet strong clustering-based defense baseline. We hope that our frameworks and benchmarks could serve as the cornerstones for future model development and evaluations.

==> analysis.tex <==
\section{Learning Analysis}

we empirically study the feature learning process through manipulating the hyper-parameters of backdoor poisoning methods to explore three different dimensions.
Specifically, we adjust the poison rate, trigger type, and attack setting (e.g. dirty or label-consistent attack), which correspond to the statistical correlation of the injected feature and the target label, xx, yy, separately.

We conduct a thorough empirical study on feature learning on three different datasets with
%LIMIT-BERT \cite{zhou2019limit} 
RoBERTa \cite{liu2019roberta} as the testbed. Our main findings are as follows: 
\begin{itemize}[topsep=1pt, partopsep=1pt, leftmargin=12pt, itemsep=-2pt]
    \item .
\end{itemize}

\subsection{Formalization}
We treat the backdoor trigger as an artificially injected pattern and employ a general framework to discuss this feature learning process. 
Specifically, we utilize the backdoor poisoning methods to get the artificially dataset $\mathbb{D}$'. 
A general feature encoder $f$ (e.g. the pretrained BERT) is fit on $\mathbb{D}$' to learn representation embeddings that are used by a linear classifier to make predictions. 
In this work, we analyze the distribution of these representation embeddings during the training time to empirically study the feature learning process. 

Without loss of generality, we use the sentiment analysis task to illustrate some basic concepts. 
Each sample $x$ from the artificially modified dataset $\mathbb{D}'$ can be denoted as $x = (x_1, x_2, x_3)$ for simplicity, where $x_i$ is the feature in $x$\footnote{This notation can be easily extended to more features.}. 
Specifically, $x_1$ denotes existence of the artificially injected pattern (e.g. a irrelevant sentence), $x_2$ denotes the sentiment irrelevant feature (e.g. function words that do not express emotion), and $x_3$ denotes the sentiment predictive feature (e.g. adjectives like good, terrible). 
We specify one class as the target class.
The paired label $y$ is directly set to the target class when the artificially injected pattern exists. 
Otherwise, it is decided by $x_3$ as in common cases. 



In our study, we adjust the construction process of $\mathbb{D}'$ to explore 3 dimensions: 
\begin{itemize}[topsep=1pt, partopsep=1pt, leftmargin=12pt, itemsep=-2pt]
    \item The statistical correlation $\alpha$ of $x_1$ and the target class, corresponding to the poison rate. 
    \item The abstraction level $\beta$ of $x_1$ that determines the learning difficulty.
    
    \item The conflict indicator $\sigma$ that denotes whether $x_3$ conflicts with the target class when $x_1$ exists, corresponding to the two attack settings. 
\end{itemize}








==> cube.tex <==
\section{Benchmark Experiments of Defenses}
To protect NLP systems from backdoor attacks, some backdoor defense models have been proposed. In this section, we first discuss the goals and accessibility of defense models (\cref{sec:defense:discuss}), categorize and discuss applicable scenarios (\cref{sec:defense_sce}).
We then propose a simple clustering-based defense model (\cref{sec:defense_cube}). Finally, we benchmark existing defense models along with our model (\cref{sec:defense_exp},\cref{sec:defense_inference}).

\subsection{Goals and Accessibility}
\label{sec:defense:discuss}
We summarize the goals and accessibility of defense models as follows:

\textbf{Goals.} Most existing defenders are detection-based~\cite{gao2021strip, Yang2021rap, chen2021bki}, which identify poisoned samples from benign ones and remove them. Correction-based methods~\cite{Qi2021onion} further modify each potentially poisoned samples to remove the triggers.

\textbf{Accessibility.} There are usually two resources available for defenders, clean datasets and poisoned models. Some works~\cite{Qi2021onion, gao2021strip, Yang2021rap} require a clean dataset to determine the thresholds for detecting suspicious samples or tokens. Backdoored models behave differently on poisoned samples and normal samples, thus utilizing a poisoned model to identify poisoned samples is also a common practice~\cite{chen2021bki, gao2021strip, Yang2021rap}.

\subsection{Defense Scenarios and Evaluation Methodologies}
\label{sec:defense_sce}
 Generally, there are two defense scenarios. \textbf{Training-time defense} aims to train clean models with poisoned datasets, such as filtering out poisoned samples~\cite{chen2021bki}. Apparently, such kind of defense methods 
only suits Scenario \uppercase\expandafter{\romannumeral1} and the changes in ASR and CACC are the most essential metrics.
\textbf{Inference-time defense} manages to prevent the backdoor in the poisoned model being triggered. %Methods of this line detect poisoned inputs by their special features like fluency~\cite{Qi2021onion} or robustness~\cite{gao2021strip, Yang2021rap}, then remove them. 
Among them, detection-based methods~\cite{gao2021strip, Yang2021rap} identify poisoned samples from benign ones and reject them, and correction-based methods~\cite{Qi2021onion} modify each potentially poisoned samples to remove the triggers. As this line of defense methods only need test samples and poisoned model, they can be applied in all three scenarios.
We can evaluate both sorts of methods with ASR and CACC after defense. Specifically for detection-based methods, we can also measure their detection performances. 


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}

\subsection{A Simple Training-time Defense Model: CUBE}
\label{sec:defense_cube}

\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-20pt}
  \begin{center}
    \includegraphics[trim=20 10 35 30, clip, width=0.42\textwidth]{figures/Visualization_badnets.pdf}
    \caption{Visualization of the last hidden states of BadNet backdoor training.}
    \label{fig:visualization}
  \end{center}
  \vspace{-10pt}
\end{wrapfigure} 


\textbf{Motivation.} Our discussion and experiments reveal that most defense methods are applied at inference-time, while training-time defense remains less explored. Moreover, current defense methods can only deal with token-level triggers, leaving syntactic and style triggers unsolved. To deal with the problems, we utilize the analysis tools in \ToolName\ to observe the dynamics of backdoor learning. Specifically, we train a BERT-base model on the BadNet-poisoned SST-2 dataset and visualize its last hidden states. In Figure~\ref{fig:visualization}, we can observe that the poison samples finally cluster together and separate from the normal clusters so that we can defend the backdoor poisoning by detecting the poison cluster and drop it.
Therefore, we propose CUBE, to perform \textbf{C}l\textbf{U}stering-based poisoned sample filtering for \textbf{B}ackdoor-fre\textbf{E} training. 

%And quantitatively, we compute the Davies Bouldin score \cite{Davies1979dbscore} (DB score, the lower the better)  to assess the separation degree of clusters. As seen in Figure \ref{fig:clustering_metrics}, the DB score drops sharply during training, indicating the potential to identify and drop the poison cluster while preserving the normal ones.

% \begin{figure}
%     \vspace{-5pt}
%      \centering
%      \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/Visualization_badnets.pdf}
%          \label{fig:visualization}
%      \end{subfigure}
%     %  \hfill
%     %  \begin{subfigure}[b]{0.49\textwidth}
%     %      \centering
%     %      \includegraphics[width=\textwidth]{figures/Clustering Metrics.pdf}
%     %      \caption{}
%     %      \label{fig:clustering_metrics}
%     %  \end{subfigure}
% \vspace{-3pt}
% \caption{Visualization of the last hidden states of BadNet backdoor training.} %The poisoned samples cluster together and separate from normal samples. 
%(b) The Davies Bouldin scores and loss values.}% The descending trend of DB score verifies that we can drop only the poisoned cluster.}
% \label{fig:cube}
% \end{figure}


\textbf{Method.} Motivated by the above idea, We propose a three-step pipeline to obtain a filtered dataset for backdoor-free training.
(1) Representation learning. At the first step, we train a model with the original dataset directly, and use this potentially backdoor-injected model to map poisoned and normal samples to the embedding space. 
%LIMIT-BERT~\cite{zhou-etal-2020-limit}, which enhances BERT~\cite{devlin-etal-2019-bert} with linguistic knowledge that helps us cope with syntactic and style triggers.
%as our encoder due to its strong representation learning ability.
%We train the model until convergence on the training dataset to better capture the discrepancy between normal and poisoned samples. 
(2) Clustering. Given the representation embeddings of all samples, we employ an advanced density clustering algorithm HDBSCAN~\cite{mcinnes2017hdbscn} to identify distinctive clusters and use UMAP \cite{NBC2020umap} to reduce the dimension of the data representation to 10-D, which brings benefits to clustering~\cite{ryan2020n2d, wu2022deep}. %we hypothesize that the poisoned samples spontaneously form a small cluster in the hidden space. To identify distinctive clusters, we employ an advanced  density clustering algorithm HDBSCAN~\cite{mcinnes2017hdbscn}. However, density-based clustering is severely affected by the sparsity of high-dimensional data, so we use UMAP \cite{NBC2020umap} to reduce the dimension of the data representation to 10-D, which brings benefits to clustering~\cite{ryan2020n2d, wu2022deep}.
(3) Filtering. After clustering, with the presumption that poisoned samples are fewer than normal samples, we keep only the largest predicted clusters for each ground-truth label and drop all other samples. Finally, we obtain the processed dataset. 

\subsection{Experiments of Training-time Defense}
\label{sec:defense_exp}
\textbf{Setup.} We validate CUBE against multiple attack methods on SST-2 with a BERT-base victim model. The poison rate is set at $0.1$. For baseline methods, besides the training-time model BKI~\cite{chen2021bki}, we also adapt three inference-time models, STRIP~\cite{gao2021strip}, ONION~\cite{Qi2021onion} and RAP~\cite{Yang2021rap}, to apply them in training-time defense. The details can be found in Appendix~\ref{app:defense_train}. 

\textbf{Results.} We present the ASR and CACC under defense in \Cref{tab:eval_cube,tab:eval_cube_hsol_ag}. It is clearly seen that CUBE could reduce the ASR nearly to the upper bounds (i.e. remove all poisoned samples and remain all clean samples), while keeping high clean accuracy. Compared with baseline models, CUBE achieves the best ASR reduction among all the models. More importantly, we highlight that CUBE can effectively defend against syntactic and style backdoor attacks, while other defense models don't work. As other baselines manage to find suspicious tokens in a sentence, they fail to defend semantic-level triggers in SynBkd and StyleBkd. Meanwhile, CUBE identifies poisoned samples in the embedding space, which is not limited by trigger types.
On clean accuracy, CUBE also gets high scores, meaning that a good balance between utility and safety is reached. 
%Oppositely, we notice that although RAP dramatically reduces the ASR of StyleBkd to $1.7\%$, the performance of the victim model is largely damaged on benign samples.  


\begin{table*}
\vspace{-1pt}
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{l|c|cc|cc|cc|cc}

\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{Defender}} & None  & \multicolumn{2}{c|}{BadNet}     & \multicolumn{2}{c|}{AddSent}    & \multicolumn{2}{c|}{SynBkd}  & \multicolumn{2}{c}{StyleBkd}    \\
\multicolumn{1}{c|}{}                          & CACC    & ASR            & CACC             & ASR            & CACC             & ASR            & CACC             & ASR            & CACC             \\ \midrule
\rowcolor{gray!40} w/o Defense                                    & 91.10 & 100.0          & 91.21          & 100.0          & 91.16          & 86.08          & 90.77          & 77.30          & 90.34          \\
ONION                                          & 91.71 & 29.93          & 88.14          & 49.78          & 91.10          & 89.25          & 89.35          & 83.37          & 85.06          \\
BKI                                            & 91.16 & \textbf{15.79} & 89.79          & 33.55          & 90.72          & 88.49          & 89.13          & 81.58          & 89.46          \\
STRIP                                          & 87.75 & 99.78          & \textbf{90.23} & 28.62          & \textbf{91.39} & 88.71          & 90.44          & 83.48          & 86.99          \\
RAP                                            & \textbf{91.93} & 90.79          & 86.71          & 27.19          & 91.71          & 93.42          & 86.49          & 84.82          & 87.15          \\
CUBE                                           & 90.66 & 15.90          & 90.17          & \textbf{24.01} & 90.28          & \textbf{45.61} & \textbf{91.32} & \textbf{22.43} & \textbf{91.27} \\
\rowcolor{gray!40} Oracle                                      & -     & 12.28          & 90.83          & 15.35          & 90.33          & 32.46          & 90.61          & 29.02          & 89.68          \\ \bottomrule
\end{tabular}
}
\caption{Evaluation results for training-time defense on SST-2. ``Oracle'' stands for removing all poisoned samples and remaining all normal samples. \textbf{Bold}: Lowest ASR and highest CACC.}
\label{tab:eval_cube}
\vspace{-5pt}
\end{table*}

\begin{table}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}c|c|cc|rr|cc|cc@{}}
\toprule
\multirow{2}{*}{Defender} & None  & \multicolumn{2}{c|}{BadNet} & \multicolumn{2}{c|}{AddSent}                        & \multicolumn{2}{c|}{SynBkd} & \multicolumn{2}{c}{StyleBkd} \\
                          & CACC  & ASR          & CACC         & \multicolumn{1}{c}{ASR} & \multicolumn{1}{c|}{CACC} & ASR            & CACC          & ASR         & CACC        \\ \midrule
\rowcolor{gray!40} w/o Defense                                    & 91.10 & 100.0          & 91.21          & 100.0          & 91.16          & 86.08          & 90.77          & 77.30          & 90.34          \\
ONION                     & 86.77 & 20.50        & 86.71        & 95.50                   & 87.31                     & 92.65          & 83.96         & 82.55       & 84.24       \\
STRIP                     & 91.49 & 94.08        & 87.37        & 97.48                   & 88.96                     & 86.40          & 88.96         & 78.35       & 90.28       \\
RAP                       & 45.74 & 91.01        & 88.69        & 45.94                   & 65.79                     & 31.58          & 88.74         & 52.12       & 51.95       \\ \bottomrule
\end{tabular}
}
\vspace{7pt}
\caption{Evaluation results for inference-time defense on SST-2.}
\vspace{-20pt}
\label{tab:inference_asr}
\end{table}

\subsection{Experiments of Inference-time Defense}
\label{sec:defense_inference}
\textbf{Setup.} As the defense performances of inference-time defenders are mainly affected by the trigger types, we benchmark them against four attack methods in Scenario \uppercase\expandafter{\romannumeral1}. We report the ASR on the poisoned test set and CACC on the clean test set. See details in Appendix~\ref{app:defense_inference}. 
%In ASR calculation, if a poisoned sample is detected, the attack fail. So we only count the poisoned samples which pass the detection and change model predictions for success attacks. And for CACC, if a normal sample is detected as poisoned, we say the model makes a wrong prediction. 

\textbf{Results.} We report benchmark experiment results for inference-time defense methods in Table \ref{tab:inference_asr} and  Appendix~\ref{app:defense_inference}. We can see that ONION can only defend against BadNet and fail on all other attackers. STRIP detects few poisoned samples and performs poorly on all datasets. Although RAP could discover most poisoned samples and reject them, this method also filters out many clean samples, damaging the utility of the victim models. Our experiments show that existing inference-time defenders are not good enough, and more efforts are urgently needed to develop effective defense algorithms.
